Mask and Reason: Pre-Training Knowledge Graph Transformers for Complex Logical Queries

Knowledge graph (KG) embeddings have been a mainstream approach for reasoning over incomplete KGs. However, limited by their inherently shallow and static architectures, they can hardly deal with the rising focus on complex logical queries, which comprise logical operators, imputed edges, multiple source entities, and unknown intermediate entities. In this work, we present the Knowledge Graph Transformer (kgTransformer) with masked pre-training and fine-tuning strategies. We design a KG triple transformation method to enable Transformer to handle KGs, which is further strengthened by the Mixture-of-Experts (MoE) sparse activation. We then formulate the complex logical queries as masked prediction and introduce a two-stage masked pre-training strategy to improve transferability and generalizability. Extensive experiments on two benchmarks demonstrate that kgTransformer can consistently outperform both KG embedding-based baselines and advanced encoders on nine in-domain and out-of-domain reasoning tasks. Additionally, kgTransformer can reason with explainability via providing the full reasoning paths to interpret given answers.

==> tables/hit1_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{tabular}{@{}ll|p{0.8cm}<{\centering}p{0.8cm}<{\centering}|p{0.8cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}@{}}
\toprule[1.2pt]
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Model}    & \multirow{2}{*}{Avg}                      & \multirow{2}{* }{\makecell[c]{Avg\\w.o. u}}                               & \multicolumn{5}{c}{In-domain}                                                                                                                                                      & \multicolumn{4}{c}{Out-of-domain}                \\ \cmidrule(l){5-9} \cmidrule(l){10-13}
\multicolumn{1}{l}{} & \multicolumn{1}{l}{}    & \multicolumn{1}{|l}{} &  & \multicolumn{1}{c}{1p} & \multicolumn{1}{c}{2p} & \multicolumn{1}{c}{3p} & \multicolumn{1}{c}{2i} & \multicolumn{1}{c}{3i} & \multicolumn{1}{c}{ip} & \multicolumn{1}{c}{pi} & \multicolumn{1}{c}{2u} & \multicolumn{1}{c}{up} \\ \midrule
\multirow{8}{*}{FB15k-237}& \multicolumn{1}{|l|}{GQE~\cite{hamilton2018embedding}}                                  & 0.103                                      & 0.250                                                & 0.346                   & 0.193                   & 0.145                   & 0.25                   & 0.355                   & 0.086                   & 0.156                   & 0.145                   & 0.151\\
                          & \multicolumn{1}{|l|}{Q2B~\cite{ren2019query2box}}                                       & -                                      & -                                               & -                 & -                    &-                  &-               & -                 & -                  &-                 & -                   & -                 \\
                          & \multicolumn{1}{|l|}{EmQL~\cite{sun2021faithful}$^1$}                                   & 0.219                                 & 0.241                                                & 0.389                           & 0.201                   & 0.154                   & 0.275                   & 0.386                   & 0.101                   & 0.184                           & 0.115                   & 0.165                  \\
                          & \multicolumn{1}{|l|}{BiQE~\cite{kotnis2021answering}}                                   & -                                          & 0.293                                                & 0.439                   & 0.281                   & 0.239                   & 0.333                   & 0.474                   & 0.110                   & 0.177                   & -                       & -                      \\
                          & \multicolumn{1}{|l|}{HypE~\cite{choudhary2021self}}                                       & 0.335                                      & 0.359                                                & 0.572                   & 0.366                   & 0.255                   & 0.399                   & 0.527                   & 0.145                   & 0.246                   & 0.225                   & 0.282                  \\
                          & \multicolumn{1}{|l|}{CQD\footnotesize{(CO)}\normalsize~\cite{arakelyan2021complex}}     & 0.272                             & 0.290                                                & 0.512                   & 0.213                   & 0.131                   & 0.352                   & 0.457                   & 0.146                   & 0.222                   & 0.281                   & 0.132                  \\
                          & \multicolumn{1}{|l|}{CQD\footnotesize{(Beam)}\normalsize~\cite{arakelyan2021complex}}   & 0.290                             & 0.315                                                & 0.512                   & 0.288                   & 0.221                   & 0.352                   & 0.457                   & 0.129                   & 0.249                   & 0.284                   & 0.121                  \\ \cmidrule{2-13}
                          & \multicolumn{1}{|l|}{\method} & \\\midrule%0.312                                      & 0.334                                                & 0.455                   & 0.306                   & 0.241                   & 0.389                   & 0.513                   & 0.165                   & 0.269                   & 0.264                   & 0.210                                 \\ \midrule
\multirow{8}{*}{NELL995}& \multicolumn{1}{|l|}{GQE~\cite{hamilton2018embedding}}                                    & 0.21                                   & 0.270                                                & 0.311                   & 0.193                   & 0.175                   & 0.273                   & 0.399                   & 0.078                   & 0.168                   & 0.159                   & 0.13                  \\
                          & \multicolumn{1}{|l|}{Q2B~\cite{ren2019query2box}}                                       & 0.254                                      & 0.317                                                & 0.413                   & 0.225                   & 0.173                   & 0.275                   & 0.378                   & 0.105                   & 0.18                   & 0.198                   & 0.178                  \\
                          & \multicolumn{1}{|l|}{EmQL~\cite{sun2021faithful}$^1$}                                   & 0.277                                      & 0.294                                                & 0.456                   & 0.231                   & 0.172                   & 0.331                   & 0.483                   & 0.143                   & 0.244                   & 0.226                   & 0.207                  \\
                          & \multicolumn{1}{|l|}{BiQE~\cite{kotnis2021answering}}                                   & \multicolumn{1}{l}{-}                      & 0.344                                                & 0.587                      & 0.305                   & 0.326                   & 0.371                   & \underline{0.531}                   & 0.103                   & 0.187                   & \multicolumn{1}{l}{-}   & \multicolumn{1}{l}{-}  \\
                          & \multicolumn{1}{|l|}{HypE~\cite{choudhary2021self}}                                       & 0.371                                      & 0.375                                                & \underline{0.618}                      & 0.359                   & 0.312                   & 0.400                   & 0.563                   & 0.143                   & 0.227                   & 0.441                   & \bf 0.278                  \\
                          & \multicolumn{1}{|l|}{CQD\footnotesize{(CO)}\normalsize~\cite{arakelyan2021complex}}     & 0.368                                      & 0.370                                                & \bf 0.667                      & 0.265                   & 0.220                   & \bf 0.410                   & 0.529                   & \underline{0.196}                   & \bf 0.302                   & \bf 0.531                   & 0.194                  \\
                          & \multicolumn{1}{|l|}{CQD\footnotesize{(Beam)}\normalsize~\cite{arakelyan2021complex}}   & \underline{0.375}                                      & \underline{0.385}                                                & \bf 0.667                   & 0.350                   & 0.288                   & \bf 0.410                   & 0.529                   & 0.171                   & 0.277                   & \bf 0.531                   & 0.156                  \\ \cmidrule{2-13}
                          & \multicolumn{1}{|l|}{\method} & \bf 0.398                                      & \bf 0.406                                                & 0.617                   & \bf 0.401                   & \bf 0.367                   & \underline{0.405}                   & \bf 0.546                   & \bf 0.203                   & \underline{0.300}                   & \underline{0.469}                   & \underline{0.270}                  \\ \bottomrule[1.2pt]
\end{tabular}

==> tables/mrr_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{tabular}{@{}ll|p{0.8cm}<{\centering}p{0.8cm}<{\centering}|p{0.8cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}@{}}
\toprule[1.2pt]
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Model}    & \multirow{2}{*}{Avg}                      & \multirow{2}{* }{\makecell[c]{Avg\\w.o. u}}                               & \multicolumn{5}{c}{In-domain}                                                                                                                                                      & \multicolumn{4}{c}{Out-of-domain}                \\ \cmidrule(l){5-9} \cmidrule(l){10-13}
\multicolumn{1}{l}{} & \multicolumn{1}{l}{}    & \multicolumn{1}{|l}{} &  & \multicolumn{1}{c}{1p} & \multicolumn{1}{c}{2p} & \multicolumn{1}{c}{3p} & \multicolumn{1}{c}{2i} & \multicolumn{1}{c}{3i} & \multicolumn{1}{c}{ip} & \multicolumn{1}{c}{pi} & \multicolumn{1}{c}{2u} & \multicolumn{1}{c}{up} \\ \midrule
\multirow{8}{*}{NELL995}& \multicolumn{1}{|l|}{GQE~\cite{hamilton2018embedding}}                                    & 0.21                                   & 0.228                                                & 0.311                   & 0.193                   & 0.175                   & 0.273                   & 0.399                   & 0.078                   & 0.168                   & 0.159                   & 0.13                  \\
                          & \multicolumn{1}{|l|}{Q2B~\cite{ren2019query2box}}                                       & 0.254                                      & 0.267                                                & 0.413                   & 0.227                   & 0.208                   & 0.288                   & 0.414                   & 0.125                   & 0.193                   & 0.266                   & 0.155                  \\
                          & \multicolumn{1}{|l|}{BiQE~\cite{kotnis2021answering}}                                   & - & -& -& -& -& -& -& -& -& -& -  \\
                          & \multicolumn{1}{|l|}{HypE~\cite{choudhary2021self}}                                       & \underline{0.310}                                      & \underline{0.316}                                                & \underline{0.460}                     & \underline{0.306}                   & \underline{0.279}                   & \underline{0.336}                   & \underline{0.486}                   & \underline{0.135}                   & \underline{0.207}                   & \underline{0.318}                   & \bf 0.264                  \\
                          & \multicolumn{1}{|l|}{CQD\footnotesize{(CO)}\normalsize~\cite{arakelyan2021complex}}     & -                                      & -                                                & -                      & -                   & -                   &  -                   & -                   & - & -                   & -                 & -                  \\
                          & \multicolumn{1}{|l|}{CQD\footnotesize{(Beam)}\normalsize~\cite{arakelyan2021complex}}   & -                                     & -                                                & -          &-                & -                   & -                 & -                   & -                 & -                   & -                & -                \\ \cmidrule{2-13}
                          & \multicolumn{1}{|l|}{\method} &  \bf	0.360   & \bf 0.367  & \bf 0.567 &	\bf 0.358 & \bf	0.333 &\bf	0.357 &	\bf 0.486 &	\bf 0.192 &\bf	0.273 &	\bf 0.416 &	\underline{0.255}         \\ \midrule
\multirow{8}{*}{FB15k-237}& \multicolumn{1}{|l|}{GQE~\cite{hamilton2018embedding}}                                  & 0.203                                      & 0.219                                                & 0.346                   & 0.193                   & 0.145                   & 0.250                   & 0.355                   & 0.086                   & 0.156                   & 0.145                   & 0.151                  \\
                          & \multicolumn{1}{|l|}{Q2B~\cite{ren2019query2box}}                                       & 0.235                                      & 0.248                                                & 0.400                   & 0.225                   & 0.173                   & 0.275                   & 0.378                   & 0.105                   & 0.180                   & 0.198                   & 0.178                  \\
                          & \multicolumn{1}{|l|}{BiQE~\cite{kotnis2021answering}}                                   & -                                          & -                                                & -                   & -                   & -                  & -                   & -                   & -                   & -                   & -                       & -                      \\
                          & \multicolumn{1}{|l|}{HypE~\cite{choudhary2021self}}                                       & \bf 0.334                                      & \bf 0.366                                                & \bf 0.490                   & \bf 0.343                   & \underline{0.237}                   & \underline{0.339}                   & \bf 0.440                   &\bf 0.305                   & \bf 0.410                   & \underline{0.186}                   &\bf 0.260                  \\
                          & \multicolumn{1}{|l|}{CQD\footnotesize{(CO)}\normalsize~\cite{arakelyan2021complex}}     & - & -& -& -& -& -& -& -& -& -& -                  \\
                          & \multicolumn{1}{|l|}{CQD\footnotesize{(Beam)}\normalsize~\cite{arakelyan2021complex}}   &  - & -& -& -& -& -& -& -& -& -& -                 \\ \cmidrule{2-13}
                          & \multicolumn{1}{|l|}{\method} &\underline{0.313}                                       & \underline{0.334}                                                & \underline{0.435}                   & \underline{0.316}                   &\bf 0.269                   &\bf 0.364                   & \bf 0.496                   & \underline{0.184}                   & \underline{0.273}                   &\bf 0.266                   & \underline{0.216} \\                               

\bottomrule[1.2pt]
\end{tabular}
